Efficient random graph matching via degree profiles

Random graph matching refers to recovering the underlying vertex correspondence between two random graphs with correlated edges; a prominent example is when the two random graphs are given by Erd\H{o}s-R\'{e}nyi graphs $G(n,\frac{d}{n})$. This can be viewed as an average-case and noisy version of the graph isomorphism problem. Under this model, the maximum likelihood estimator is equivalent to solving the intractable quadratic assignment problem. This work develops an $\tilde{O}(n d^2+n^2)$-time algorithm which perfectly recovers the true vertex correspondence with high probability, provided that the average degree is at least $d = \Omega(\log^2 n)$ and the two graphs differ by at most $\delta = O( \log^{-2}(n) )$ fraction of edges. For dense graphs and sparse graphs, this can be improved to $\delta = O( \log^{-2/3}(n) )$ and $\delta = O( \log^{-2}(d) )$ respectively, both in polynomial time. The methodology is based on appropriately chosen distance statistics of the degree profiles (empirical distribution of the degrees of neighbors). Before this work, the best known result achieves $\delta=O(1)$ and $n^{o(1)} \leq d \leq n^c$ for some constant $c$ with an $n^{O(\log n)}$-time algorithm \cite{barak2018nearly} and $\delta=\tilde O((d/n)^4)$ and $d = \tilde{\Omega}(n^{4/5})$ with a polynomial-time algorithm \cite{dai2018performance}.

==> ack.tex <==
J.~Ding is supported in part by the NSF Grant DMS-1757479 and an Alfred Sloan fellowship.
Z.~Ma is supported in part by an NSF CAREER award DMS-1352060 and an Alfred Sloan fellowship.
Y.~Wu is supported in part by the NSF Grant CCF-1527105, an NSF CAREER award CCF-1651588, and an Alfred Sloan fellowship.
J.~Xu is supported by the NSF Grants CCF-1755960 and IIS-1838124.

J.~Ding and Y.~Wu would like to thank the Centre de Recherches Math\'ematiques at the Universit\'e de Montr\'eal, where some of the work was carried out during the Workshop on Combinatorial Statistics.
Y.~Wu is also grateful to David Pollard for helpful discussions on small ball probability.
J.~Xu would like to thank Nadav Dym  and Shahar Kovalsky for pointing out the connections between
fractional isomorphism and iterated degree sequences. 


